Work Stealing with latency

We study in this paper the impact of communication latency on the classical Work Stealing load balancing algorithm. Our approach considers existing performance models and the underlying algorithms. We introduce a latency parameter in the model and study its overall impact by careful observations of simulation results. Using this method we are able to derive a new expression of the expected running time of divisible load applications. This expression enables us to predict under which conditions a given run will yield acceptable performance. For instance, we can easily calibrate the maximal number of processors one should use for a given work platform combination. We also consider the impact of several algorithmic variants like simultaneous transfers of work or thresholds for avoiding useless transfers. All our results are validated through simulation on a wide range of parameters.

==> bibliography.tex <==
\begin{thebibliography}{2}

	\bibitem{MCMCA}  *
		N. Hamid, R. J. Walters, G.B. Wills. \textit{An analytical model of multi-core multi-cluster architecture (MCMCA)}. Open Journal of Cloud Computing(OJCC) 2(1), pp. 1-12. 2015
		
	\bibitem{Agrawal} *
		K. Agrawal, C. E. Leiserson and J. Sukha. \textit{Executing task graphs using work-stealing}. IEEE International Symposium on Parallel \& Distributed Processing (IPDPS), Atlanta, GA, pp. 1-12. 2010,
		
	\bibitem{Gast2010} *
		 N. Gast and G. Bruno. \textit{A mean field model of work stealing in large-scale systems}. In Proceedings of the ACM SIGMETRICS international conference on Measurement and modeling of computer systems (SIGMETRICS '10). ACM, New York, NY, USA, pp. 13-24. 2010
	
	\bibitem{Denis2013} *
		M.  Tchiboukdjian, N. Gast, and D. Trystram. \textit{Decentralized list scheduling}. Annals of Operations Research (2013) pp. 207-237. 2013.
	
	\bibitem{MultiCoreClusterArchitectur2015} * 
		N. Hamid, R. Walters and G. Wills, \textit{Simulation and Mathematical Analysis of Multi-core Cluster Architecture}. x17th UKSim-AMSS International Conference on Modelling and Simulation (UKSim), Cambridge, pp. 476-481. 2015.
		
	\bibitem{Leiserson1998} * 
		 M. Frigo, C. E. Leiserson, and K. H. Randall. \textit{The implementation of the Cilk-5 multithreaded language}. In Proceedings of the ACM SIGPLAN conference on Programming language design and implementation (PLDI '98), A. Michael Berman (Ed.). ACM, New York, NY, USA, pp. 212-223. 1998. 
		 
	\bibitem{Leiserson2009} * 
		 C. E. Leiserson. \textit{The Cilk++ concurrency platform}. In Proceedings of the 46th Annual Design Automation Conference , DAC 09, pp. 522-527, New York, NY, USA, ACM, 2009.
		 	
	\bibitem{Robison2008} * 
		 A. Robison, M. Voss and A. Kukanov, \textit{Optimization via Reflection on Work Stealing in TBB}. 2008 IEEE International Symposium on Parallel and Distributed Processing, Miami, FL, pp. 1-8, 2008
		 
	\bibitem{Kaapi2007} * 
		  T. Gautier, X. Besseron, L. Pigeon  \textit{KAAPI: A thread scheduling runtime system for data flow computations on cluster of multi-processors}. In Proceedings of the 2007 international workshop on Parallel symbolic computation (PASCO). ACM, New York, NY, USA, pp. 15-23, 2007
		  	
	\bibitem{Blumofe1999} *
		 R.D. Blumofe , C.E. Leiserson \textit{Scheduling multithreaded computations by work stealing}. Journal of the ACM 46(5), pp. 720–748, 1999
	
	\bibitem{Arora2001}*
		 N. S. Arora , R. D.Blumofe, C. G. Plaxton \textit{Thread scheduling for multiprogrammed multiprocessors}. Theory of Computing Systems 34(2), pp. 115–144, 2001
	

	\bibitem{Bender2002} * 
		 M. A. Bender,M. O. Rabin \textit{Online scheduling of parallel programs on heterogeneous systems with applications to cilk}. Theory of Computing Systems Special Issue on SPAA 35 p.2002 , 2002
	
	\bibitem{Sanders1999} * 
		 P. Sanders \textit{Asynchronous random polling dynamic load balancing}. In Proceedings of Algorithms and Computation: 10th International Symposium, ISAAC'99 Chennai, India  ISAAC, Springer, Lecture Notes in Computer Science, 1741, pp. 37–48 1999
	\bibitem{Berenbrink2003}*
		 P. Berenbrink, T. Friedetzky, L. A. Goldberg \textit{The natural work-stealing algorithm is stable}. SIAM Journal of Computing 32(5) pp. 1260–1279, 2003
	
	\bibitem{Mitzenmache1998} * 
		 M. Mitzenmacher \textit{Analyses of load stealing models based on differential equations}. In Proceedings of the tenth annual ACM symposium on Parallel algorithms and architectures (SPAA). ACM, New York, NY, USA, pp. 212–221, 1998
	
	\bibitem{Lueling1993} *
		 R. Lueling, B. Monien \textit{A dynamic distributed load balancing algorithm with provable good performance}. In Proceedings of the fifth annual ACM symposium on Parallel algorithms and architectures (SPAA). ACM, New York, NY, USA, pp. 164-172, 1993
	
	\bibitem{Rudolph1991} * 
		 L. Rudolph, M. Slivkin-Allalouf,E. Upfal \textit{A simple load balancing scheme for task allocation in parallel machines}. In Proceedings of the third annual ACM symposium on Parallel algorithms and architectures (SPAA). ACM, New York, NY, USA, pp. 237-245, 1991
	
	\bibitem{Muller2106} *
		S. K. Muller and A. A. Umut. \textit{Latency-Hiding Work Stealing: Scheduling Interacting Parallel Computations with Work Stealing}. In Proceedings of the 28th ACM Symposium on Parallelism in Algorithms and Architectures (SPAA). ACM, New York, NY, USA, pp. 71-82. 2016 
	 
	 \bibitem{Shigang2013} *
		 Li. Shigang, Hu. Jingyuan,C. Xin, and Z. Chongchong. \textit{Asynchronous Work Stealing on Distributed Memory Systems}. In Proceedings of the 2013 21st Euromicro International Conference on Parallel, Distributed, and Network-Based Processing (PDP). IEEE Computer Society, Washington, DC, USA, pp. 198-202. 2013
		  
	 \bibitem{swann2014} * 
		 S. Perarneau, and M. Sato. \textit{Victim Selection and Distributed Work Stealing Performance: A Case Study}. In Proceedings of the 2014 IEEE 28th International Parallel and Distributed Processing Symposium (IPDPS). IEEE Computer Society, Washington, DC, USA, pp. 659-668. 2014
		  
	 \bibitem{Seung-Jai2011} * 
		 M. Seung-Jai, I. Costin, and Y. Katherine. \textit{Hierarchical workstealing on manycore clusters}. In Fifth Conference on Partitioned Global Address Space Programming Models. Galveston Island. 2011
		 
	 \bibitem{JeanLouisRoch2006} * 
		 C. Van-Dat, J. G. Dumas, T. Gautier, G. Huard, B. Raffin, C. Rapine, and J. L. Roch Denis Trystram. \textit{Adaptive algorithms: theory and application}. In SIAM PP'06, editor, SIAM Parallel Processing, Mini-Symposium MS1: Adaptive algorithms for scientific computing, San Francisco, USA, February, pp. 49-50, 2006
	
	\bibitem{Hoefler2011} * 
		T.  Hoefler and M. Snir, \textit{Generic Topology Mapping Strategies for Large-Scale  Parallel  Architectures}. In Proceedings of the international conference on Supercomputing (ICS). ACM, New York, NY, USA, pp. 75-84. 2011
		
	\bibitem{Bhatele2008} * 
	
		A.  Bhatel\'e and L. V. Kal\'e, \textit{Benefits of Topology Aware Mapping for Mesh Interconnects}. Parallel Processing Letters, (Special issue on Large-Scale Parallel Processing) vol. 18, no. 4, pp. 549–566, 2008.
	
	\bibitem{Cheriere2016} * 
		N Cheriere, “SRC10. \textit{Design and Evaluation of Topology-Aware Scatter and AllGather Algorithms for Dragonfly Networks}. In Proceedings of the ACM Student Research Competition Poster of conference on Supercomputing. 2016.
	
	\bibitem{Dinan2009} * 
		J. Dinan, D. B. Larkins, P. Sadayappan, S. Krishnamoorthy, and J. Nieplocha, \textit{Scalable Work Stealing}. In Proceedings of the Conference on High Performance Computing Networking, Storage and Analysis, SC’09, New York, NY, USA, pp. 1-11, 2009.
	
	\bibitem{Gue2010} * 
		Y. Guo, J. Zhao, V. Cave, and V. Sarkar. \textit{SLAW: A scalable locality	aware adaptive work-stealing scheduler}. In Proceedings of the 15th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming (PPoPP '10). New York, USA, pp. 341-342, 2010.
		
	\bibitem{CosnardTrystram92} *
		M. Cosnard and D. Trystram, \textit{Parallel algorithms and architectures}, publisher  in International Thomson, 1995
	
	\
\end{thebibliography}

